Privacy Preserving Federated Learning with Convolutional Variational Bottlenecks

Gradient inversion attacks are an ubiquitous threat in federated learning as they exploit gradient leakage to reconstruct supposedly private training data. Recent work has proposed to prevent gradient leakage without loss of model utility by incorporating a PRivacy EnhanCing mODulE (PRECODE) based on variational modeling. Without further analysis, it was shown that PRECODE successfully protects against gradient inversion attacks. In this paper, we make multiple contributions. First, we investigate the effect of PRECODE on gradient inversion attacks to reveal its underlying working principle. We show that variational modeling introduces stochasticity into the gradients of PRECODE and the subsequent layers in a neural network. The stochastic gradients of these layers prevent iterative gradient inversion attacks from converging. Second, we formulate an attack that disables the privacy preserving effect of PRECODE by purposefully omitting stochastic gradients during attack optimization. To preserve the privacy preserving effect of PRECODE, our analysis reveals that variational modeling must be placed early in the network. However, early placement of PRECODE is typically not feasible due to reduced model utility and the exploding number of additional model parameters. Therefore, as a third contribution, we propose a novel privacy module -- the Convolutional Variational Bottleneck (CVB) -- that can be placed early in a neural network without suffering from these drawbacks. We conduct an extensive empirical study on three seminal model architectures and six image classification datasets. We find that all architectures are susceptible to gradient leakage attacks, which can be prevented by our proposed CVB. Compared to PRECODE, we show that our novel privacy module requires fewer trainable parameters, and thus computational and communication costs, to effectively preserve privacy.

==> tables/apx/ablation_apx_beta.tex <==
\begin{table*}
\centering
\caption{ApxBeta}
\label{tab:apx_beta}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\toprule
 &  &  &  & Metric & SSIM $\downarrow$ & ASR [\%] $\downarrow$ & PSNR $\downarrow$ & MSE $\uparrow$ & LPIPS $\uparrow$ & Accuracy [\%] $\uparrow$ \\
Defense & $P$ & $s_E$ & $k_E$ & $\beta$ &  &  &  &  &  &  \\
\midrule
None & - & - & - & - & {\cellcolor[HTML]{E0422F}} \color[HTML]{F1F1F1} \itshape 0.87 ($\pm$0.11) & {\cellcolor[HTML]{B30D26}} \color[HTML]{F1F1F1} \itshape 96.88 & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 21.09 ($\pm$2.88) & {\cellcolor[HTML]{CE2827}} \color[HTML]{F1F1F1} \itshape 0.01 ($\pm$0.01) & {\cellcolor[HTML]{FDC171}} \color[HTML]{000000} \itshape 0.20 ($\pm$0.09) & {\cellcolor[HTML]{CBE982}} \color[HTML]{000000} \itshape 62.53 ($\pm$0.16) \\
\midrule
\multirow[c]{5}{*}{CVB} & \multirow[c]{5}{*}{0} & \multirow[c]{5}{*}{$\frac{1}{2}$} & \multirow[c]{5}{*}{5} & $10^{-1}$ & {\cellcolor[HTML]{6BBF64}} \color[HTML]{000000} 0.21 ($\pm$0.07) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{ECF7A6}} \color[HTML]{000000} \bfseries 9.51 ($\pm$1.49) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.12 ($\pm$0.04) & {\cellcolor[HTML]{04703B}} \color[HTML]{F1F1F1} 0.58 ($\pm$0.06) & {\cellcolor[HTML]{39A758}} \color[HTML]{F1F1F1} \bfseries 67.17 ($\pm$0.58) \\
 &  &  &  & $10^{-2}$ & {\cellcolor[HTML]{5DB961}} \color[HTML]{F1F1F1} \bfseries 0.19 ($\pm$0.07) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{F1F9AC}} \color[HTML]{000000} 9.75 ($\pm$1.36) & {\cellcolor[HTML]{15904C}} \color[HTML]{F1F1F1} 0.11 ($\pm$0.04) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.59 ($\pm$0.06) & {\cellcolor[HTML]{87CB67}} \color[HTML]{000000} 64.97 ($\pm$0.19) \\
 &  &  &  & $10^{-3}$ & {\cellcolor[HTML]{5DB961}} \color[HTML]{F1F1F1} \bfseries 0.19 ($\pm$0.07) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{FBFDBA}} \color[HTML]{000000} 10.34 ($\pm$1.12) & {\cellcolor[HTML]{4BB05C}} \color[HTML]{F1F1F1} 0.10 ($\pm$0.02) & {\cellcolor[HTML]{04703B}} \color[HTML]{F1F1F1} 0.58 ($\pm$0.06) & {\cellcolor[HTML]{B1DE71}} \color[HTML]{000000} 63.55 ($\pm$0.50) \\
 &  &  &  & $10^{-4}$ & {\cellcolor[HTML]{66BD63}} \color[HTML]{F1F1F1} 0.20 ($\pm$0.07) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{FBFDBA}} \color[HTML]{000000} 10.32 ($\pm$1.25) & {\cellcolor[HTML]{4BB05C}} \color[HTML]{F1F1F1} 0.10 ($\pm$0.03) & {\cellcolor[HTML]{04703B}} \color[HTML]{F1F1F1} 0.58 ($\pm$0.06) & {\cellcolor[HTML]{B7E075}} \color[HTML]{000000} 63.31 ($\pm$0.54) \\
 &  &  &  & $10^{-5}$ & {\cellcolor[HTML]{6BBF64}} \color[HTML]{000000} 0.21 ($\pm$0.07) & {\cellcolor[HTML]{016A38}} \color[HTML]{F1F1F1} 0.78 & {\cellcolor[HTML]{FDFEBC}} \color[HTML]{000000} 10.43 ($\pm$1.24) & {\cellcolor[HTML]{84CA66}} \color[HTML]{000000} 0.09 ($\pm$0.03) & {\cellcolor[HTML]{08773F}} \color[HTML]{F1F1F1} 0.57 ($\pm$0.07) & {\cellcolor[HTML]{B1DE71}} \color[HTML]{000000} 63.56 ($\pm$0.66) \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/apx/ablation_apx_channels.tex <==
\begin{table*}
\centering
\caption{ApxChannels}
\label{tab:apx_channels}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\toprule
 &  &  &  & Metric & SSIM $\downarrow$ & ASR [\%] $\downarrow$ & PSNR $\downarrow$ & MSE $\uparrow$ & LPIPS $\uparrow$ & Accuracy [\%] $\uparrow$ \\
Defense & $P$ & $s_E$ & $k_E$ & $\beta$ &  &  &  &  &  &  \\
\midrule
None & - & - & - & - & {\cellcolor[HTML]{E0422F}} \color[HTML]{F1F1F1} \itshape 0.87 ($\pm$0.11) & {\cellcolor[HTML]{B30D26}} \color[HTML]{F1F1F1} \itshape 96.88 & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 21.09 ($\pm$2.88) & {\cellcolor[HTML]{C82227}} \color[HTML]{F1F1F1} \itshape 0.01 ($\pm$0.01) & {\cellcolor[HTML]{FDB96A}} \color[HTML]{000000} \itshape 0.20 ($\pm$0.09) & {\cellcolor[HTML]{CBE982}} \color[HTML]{000000} 62.53 ($\pm$0.16) \\
\midrule
\multirow[c]{6}{*}{CVB} & \multirow[c]{6}{*}{0} & $\frac{1}{2}$ & 5 & $10^{-1}$ & {\cellcolor[HTML]{6BBF64}} \color[HTML]{000000} 0.21 ($\pm$0.07) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{ECF7A6}} \color[HTML]{000000} 9.51 ($\pm$1.49) & {\cellcolor[HTML]{39A758}} \color[HTML]{F1F1F1} 0.12 ($\pm$0.04) & {\cellcolor[HTML]{108647}} \color[HTML]{F1F1F1} 0.58 ($\pm$0.06) & {\cellcolor[HTML]{39A758}} \color[HTML]{F1F1F1} 67.17 ($\pm$0.58) \\
 &  & 2 & 5 & $10^{-1}$ & {\cellcolor[HTML]{199750}} \color[HTML]{F1F1F1} \bfseries 0.10 ($\pm$0.06) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{DDF191}} \color[HTML]{000000} 8.70 ($\pm$1.51) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.14 ($\pm$0.05) & {\cellcolor[HTML]{04703B}} \color[HTML]{F1F1F1} 0.61 ($\pm$0.06) & {\cellcolor[HTML]{FBA35C}} \color[HTML]{000000} \itshape 55.63 ($\pm$0.39) \\
 &  & 4 & 5 & $10^{-1}$ & {\cellcolor[HTML]{3FAA59}} \color[HTML]{F1F1F1} 0.15 ($\pm$0.06) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{DCF08F}} \color[HTML]{000000} \bfseries 8.59 ($\pm$1.17) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.14 ($\pm$0.04) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.62 ($\pm$0.06) & {\cellcolor[HTML]{7DC765}} \color[HTML]{000000} 65.24 ($\pm$0.31) \\
 &  & 16 & 5 & $10^{-1}$ & {\cellcolor[HTML]{A5D86A}} \color[HTML]{000000} 0.30 ($\pm$0.08) & {\cellcolor[HTML]{036E3A}} \color[HTML]{F1F1F1} 1.56 & {\cellcolor[HTML]{FFF0A6}} \color[HTML]{000000} 11.60 ($\pm$1.83) & {\cellcolor[HTML]{E3F399}} \color[HTML]{000000} 0.08 ($\pm$0.03) & {\cellcolor[HTML]{48AE5C}} \color[HTML]{F1F1F1} 0.52 ($\pm$0.06) & {\cellcolor[HTML]{18954F}} \color[HTML]{F1F1F1} 68.05 ($\pm$0.63) \\
 &  & 32 & 5 & $10^{-1}$ & {\cellcolor[HTML]{CFEB85}} \color[HTML]{000000} 0.38 ($\pm$0.11) & {\cellcolor[HTML]{2DA155}} \color[HTML]{F1F1F1} 12.50 & {\cellcolor[HTML]{FECC7B}} \color[HTML]{000000} 13.45 ($\pm$1.80) & {\cellcolor[HTML]{FECA79}} \color[HTML]{000000} 0.05 ($\pm$0.03) & {\cellcolor[HTML]{8CCD67}} \color[HTML]{000000} 0.46 ($\pm$0.07) & {\cellcolor[HTML]{0F8446}} \color[HTML]{F1F1F1} 68.79 ($\pm$1.32) \\
 &  & 64 & 5 & $10^{-1}$ & {\cellcolor[HTML]{E8F59F}} \color[HTML]{000000} 0.44 ($\pm$0.10) & {\cellcolor[HTML]{8ECF67}} \color[HTML]{000000} 26.56 & {\cellcolor[HTML]{FDB163}} \color[HTML]{000000} 14.59 ($\pm$1.76) & {\cellcolor[HTML]{FCA55D}} \color[HTML]{000000} 0.04 ($\pm$0.02) & {\cellcolor[HTML]{B1DE71}} \color[HTML]{000000} 0.42 ($\pm$0.07) & {\cellcolor[HTML]{0D8044}} \color[HTML]{F1F1F1} \bfseries 68.93 ($\pm$0.58) \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/apx/ablation_apx_kernel.tex <==
\begin{table*}
\centering
\caption{ApxKernel}
\label{tab:apx_kernel}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\toprule
 &  &  &  & Metric & SSIM $\downarrow$ & ASR [\%] $\downarrow$ & PSNR $\downarrow$ & MSE $\uparrow$ & LPIPS $\uparrow$ & Accuracy [\%] $\uparrow$ \\
Defense & $P$ & $s_E$ & $k_E$ & $\beta$ &  &  &  &  &  &  \\
\midrule
None & - & - & - & - & {\cellcolor[HTML]{E0422F}} \color[HTML]{F1F1F1} \itshape 0.87 ($\pm$0.11) & {\cellcolor[HTML]{B30D26}} \color[HTML]{F1F1F1} \itshape 96.88 & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 21.09 ($\pm$2.88) & {\cellcolor[HTML]{CE2827}} \color[HTML]{F1F1F1} \itshape 0.01 ($\pm$0.01) & {\cellcolor[HTML]{FDC574}} \color[HTML]{000000} \itshape 0.20 ($\pm$0.09) & {\cellcolor[HTML]{CBE982}} \color[HTML]{000000} 62.53 ($\pm$0.16) \\
\midrule
\multirow[c]{4}{*}{CVB} & \multirow[c]{4}{*}{0} & \multirow[c]{4}{*}{$\frac{1}{2}$} & 2 & $10^{-1}$ & {\cellcolor[HTML]{30A356}} \color[HTML]{F1F1F1} \bfseries 0.13 ($\pm$0.06) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{F2FAAE}} \color[HTML]{000000} 9.82 ($\pm$1.45) & {\cellcolor[HTML]{15904C}} \color[HTML]{F1F1F1} 0.11 ($\pm$0.04) & {\cellcolor[HTML]{0D8044}} \color[HTML]{F1F1F1} 0.55 ($\pm$0.06) & {\cellcolor[HTML]{D9EF8B}} \color[HTML]{000000} \itshape 62.01 ($\pm$1.66) \\
 &  &  & 3 & $10^{-1}$ & {\cellcolor[HTML]{5DB961}} \color[HTML]{F1F1F1} 0.19 ($\pm$0.07) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{F5FBB2}} \color[HTML]{000000} 9.97 ($\pm$1.48) & {\cellcolor[HTML]{15904C}} \color[HTML]{F1F1F1} 0.11 ($\pm$0.04) & {\cellcolor[HTML]{0D8044}} \color[HTML]{F1F1F1} 0.55 ($\pm$0.06) & {\cellcolor[HTML]{69BE63}} \color[HTML]{F1F1F1} 65.88 ($\pm$1.11) \\
 &  &  & 5 & $10^{-1}$ & {\cellcolor[HTML]{6BBF64}} \color[HTML]{000000} 0.21 ($\pm$0.07) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{ECF7A6}} \color[HTML]{000000} \bfseries 9.51 ($\pm$1.49) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.12 ($\pm$0.04) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.58 ($\pm$0.06) & {\cellcolor[HTML]{39A758}} \color[HTML]{F1F1F1} 67.17 ($\pm$0.58) \\
 &  &  & 7 & $10^{-1}$ & {\cellcolor[HTML]{78C565}} \color[HTML]{000000} 0.23 ($\pm$0.08) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{F5FBB2}} \color[HTML]{000000} 10.03 ($\pm$1.56) & {\cellcolor[HTML]{15904C}} \color[HTML]{F1F1F1} 0.11 ($\pm$0.04) & {\cellcolor[HTML]{04703B}} \color[HTML]{F1F1F1} 0.57 ($\pm$0.06) & {\cellcolor[HTML]{16914D}} \color[HTML]{F1F1F1} \bfseries 68.23 ($\pm$0.19) \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/apx/ablation_apx_position.tex <==
\begin{table*}
\centering
\caption{ApxPosition}
\label{tab:apx_position}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\toprule
 &  &  &  & Metric & SSIM $\downarrow$ & ASR [\%] $\downarrow$ & PSNR $\downarrow$ & MSE $\uparrow$ & LPIPS $\uparrow$ & Accuracy [\%] $\uparrow$ \\
Defense & $P$ & $s_E$ & $k_E$ & $\beta$ &  &  &  &  &  &  \\
\midrule
None & - & - & - & - & {\cellcolor[HTML]{E0422F}} \color[HTML]{F1F1F1} \itshape 0.87 ($\pm$0.11) & {\cellcolor[HTML]{B30D26}} \color[HTML]{F1F1F1} \itshape 96.88 & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 21.09 ($\pm$2.88) & {\cellcolor[HTML]{D22B27}} \color[HTML]{F1F1F1} \itshape 0.01 ($\pm$0.01) & {\cellcolor[HTML]{FDC574}} \color[HTML]{000000} \itshape 0.20 ($\pm$0.09) & {\cellcolor[HTML]{CBE982}} \color[HTML]{000000} 62.53 ($\pm$0.16) \\
\midrule
\multirow[c]{7}{*}{CVB} & 2 & $\frac{1}{2}$ & 3 & $10^{-1}$ & {\cellcolor[HTML]{30A356}} \color[HTML]{F1F1F1} 0.13 ($\pm$0.06) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{F2FAAE}} \color[HTML]{000000} \bfseries 9.82 ($\pm$1.45) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.11 ($\pm$0.04) & {\cellcolor[HTML]{0D8044}} \color[HTML]{F1F1F1} 0.55 ($\pm$0.06) & {\cellcolor[HTML]{D9EF8B}} \color[HTML]{000000} 62.01 ($\pm$1.66) \\
 & 3 & $\frac{1}{2}$ & 3 & $10^{-1}$ & {\cellcolor[HTML]{7FC866}} \color[HTML]{000000} 0.24 ($\pm$0.09) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{F5FBB2}} \color[HTML]{000000} 10.05 ($\pm$1.38) & {\cellcolor[HTML]{17934E}} \color[HTML]{F1F1F1} 0.10 ($\pm$0.03) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.58 ($\pm$0.08) & {\cellcolor[HTML]{82C966}} \color[HTML]{000000} \bfseries 65.10 ($\pm$1.11) \\
 & 3 & $\frac{1}{2}$ & 3 & $10^{-1}$ & {\cellcolor[HTML]{EFF8AA}} \color[HTML]{000000} 0.46 ($\pm$0.17) & {\cellcolor[HTML]{F7FCB4}} \color[HTML]{000000} 47.66 & {\cellcolor[HTML]{FED27F}} \color[HTML]{000000} 13.19 ($\pm$2.60) & {\cellcolor[HTML]{EEF8A8}} \color[HTML]{000000} 0.06 ($\pm$0.03) & {\cellcolor[HTML]{51B35E}} \color[HTML]{F1F1F1} 0.48 ($\pm$0.10) & {\cellcolor[HTML]{A7D96B}} \color[HTML]{000000} 63.93 ($\pm$0.59) \\
 & (1,2) & $\frac{1}{2}$ & 3 & $10^{-1}$ & {\cellcolor[HTML]{30A356}} \color[HTML]{F1F1F1} 0.13 ($\pm$0.07) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{FFF8B4}} \color[HTML]{000000} 10.96 ($\pm$1.73) & {\cellcolor[HTML]{57B65F}} \color[HTML]{F1F1F1} 0.09 ($\pm$0.04) & {\cellcolor[HTML]{279F53}} \color[HTML]{F1F1F1} 0.51 ($\pm$0.06) & {\cellcolor[HTML]{D9EF8B}} \color[HTML]{000000} 61.96 ($\pm$1.19) \\
 & (1,3) & $\frac{1}{2}$ & 3 & $10^{-1}$ & {\cellcolor[HTML]{279F53}} \color[HTML]{F1F1F1} \bfseries 0.12 ($\pm$0.07) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{FDFEBC}} \color[HTML]{000000} 10.45 ($\pm$1.79) & {\cellcolor[HTML]{17934E}} \color[HTML]{F1F1F1} 0.10 ($\pm$0.05) & {\cellcolor[HTML]{16914D}} \color[HTML]{F1F1F1} 0.53 ($\pm$0.05) & {\cellcolor[HTML]{EFF8AA}} \color[HTML]{000000} \itshape 60.79 ($\pm$0.53) \\
 & (2,3) & $\frac{1}{2}$ & 3 & $10^{-1}$ & {\cellcolor[HTML]{78C565}} \color[HTML]{000000} 0.23 ($\pm$0.10) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{FFFCBA}} \color[HTML]{000000} 10.75 ($\pm$1.43) & {\cellcolor[HTML]{57B65F}} \color[HTML]{F1F1F1} 0.09 ($\pm$0.03) & {\cellcolor[HTML]{04703B}} \color[HTML]{F1F1F1} 0.57 ($\pm$0.06) & {\cellcolor[HTML]{84CA66}} \color[HTML]{000000} 65.05 ($\pm$0.36) \\
 & (1,2,3) & $\frac{1}{2}$ & 3 & $10^{-1}$ & {\cellcolor[HTML]{36A657}} \color[HTML]{F1F1F1} 0.14 ($\pm$0.09) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0.00 & {\cellcolor[HTML]{FEEDA1}} \color[HTML]{000000} 11.78 ($\pm$2.08) & {\cellcolor[HTML]{C7E77F}} \color[HTML]{000000} 0.07 ($\pm$0.04) & {\cellcolor[HTML]{279F53}} \color[HTML]{F1F1F1} 0.51 ($\pm$0.06) & {\cellcolor[HTML]{EFF8AA}} \color[HTML]{000000} 60.80 ($\pm$0.66) \\
\bottomrule
\end{tabular}
\end{table*}

